REaLTabFormer: Generating Realistic Relational and Tabular Data using Transformers

Tabular data is a common form of organizing data. Multiple models are available to generate synthetic tabular datasets where observations are independent, but few have the ability to produce relational datasets. Modeling relational data is challenging as it requires modeling both a "parent" table and its relationships across tables. We introduce REaLTabFormer (Realistic Relational and Tabular Transformer), a tabular and relational synthetic data generation model. It first creates a parent table using an autoregressive GPT-2 model, then generates the relational dataset conditioned on the parent table using a sequence-to-sequence (Seq2Seq) model. We implement target masking to prevent data copying and propose the $Q_{\delta}$ statistic and statistical bootstrapping to detect overfitting. Experiments using real-world datasets show that REaLTabFormer captures the relational structure better than a baseline model. REaLTabFormer also achieves state-of-the-art results on prediction tasks, "out-of-the-box", for large non-relational datasets without needing fine-tuning.

==> REaLTabFormer ArXiv/tables/data_summary.tex <==
% Data Summary
\begin{table*}[t]
\caption{Summary of the datasets used in the experiments for non-relational tabular data.}
\label{tab:data-summary}
\vskip 0.1in
\begin{center}
\begin{small}
    \begin{tabular}{lcccccccc}
        \toprule
        Abbr & Name & \# Train & \# Validation & \# Test & \# Num & \# Cat & Task type \\
        \midrule
        AB & Abalone & $2672$ & $669$ & $836$ & $7$ & $1$ & Regression \\
        AD & Adult ROC & $26048$ & $6513$ & $16281$ & $6$ & $8$ & Binclass \\
        BU & Buddy & $12053$ & $3014$ & $3767$ & $4$ & $5$ & Multiclass \\
        CA & California Housing & $13209$ & $3303$ & $4128$ & $8$ & $0$ & Regression \\
        DI & Diabetes & $491$ & $123$ & $154$ & $8$ & $0$ & Binclass \\
        FB & Facebook Comments Volume & $157638$ & $19722$ & $19720$ & $50$ & $1$ & Regression  \\
        \bottomrule
    \end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}




==> REaLTabFormer ArXiv/tables/relational_ld_logistic_results.tex <==
\begin{table}[t]
\caption{Logistic detection measure for the generated parent, child, and merged tables by the Hierarchical Modeling Algorithm (HMA) from SDV and the REaLTabFormer (RTF) models. This uses the logistic regression model as the detector.}
\label{tab:relational-ld-logistic-results}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\toprule
Dataset & Table & SDV & RTF \\
\midrule

\multirow{3}{*}{ Rossmann } &

Parent &
\wstd{78.67}{6.79} & % SDV
\wstd{92.75}{4.28} \\ & % REaLTabFormer

Child &
\wstd{16.62}{0.86} & % SDV
\wstd{59.00}{2.92} \\ & % REaLTabFormer

Merged &
\wstd{12.00}{0.73} & % SDV
\wstd{50.69}{2.41} \\ % REaLTabFormer

\midrule

\multirow{3}{*}{ Airbnb } &

Parent &
\wstd{98.66}{1.34} & % SDV
\wstd{99.68}{0.38} \\ & % REaLTabFormer

Child &
\wstd{0.00}{0.00} & % SDV
\wstd{26.33}{0.78} \\ & % REaLTabFormer


Merged &
\wstd{96.71}{2.79} & % SDV
\wstd{98.93}{0.82} \\ % REaLTabFormer

% \midrule

% \multirow{3}{*}{
% Telstra } &

% Parent &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ & % REaLTabFormer

% Child &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ & % REaLTabFormer


% Merged &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ % REaLTabFormer

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> REaLTabFormer ArXiv/tables/relational_ld_results.tex <==
\begin{table}[t]
\caption{Logistic detection (LD) measure using random forest model for the generated parent, child, and merged tables by the Hierarchical Modeling Algorithm (HMA) from SDV and the REaLTabFormer (RTF) models. Our model consistently beats the SDV model on this metric.}
\label{tab:relational-ld-results}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccc}
\toprule
Dataset & Table & SDV & RTF \\
\midrule
\multirow{3}{*}{ Rossmann } &

Parent &
\wstd{31.77}{3.41} & % SDV
\textbf{ \wstd{81.04}{4.54} } \\ & % REaLTabFormer

Child &
\wstd{6.53}{0.39} & % SDV
\textbf{ \wstd{52.08}{0.89} } \\ & % REaLTabFormer

Merged &
\wstd{2.80}{0.25} & % SDV
\textbf{ \wstd{28.33}{2.31} } \\ % REaLTabFormer

\midrule

\multirow{3}{*}{ Airbnb } &

Parent &
\wstd{7.37}{0.72} & % SDV
\textbf{ \wstd{89.65}{1.92} } \\ & % REaLTabFormer

Child &
\wstd{0.00}{0.00} & % SDV
\textbf{ \wstd{30.48}{0.79} } \\ & % REaLTabFormer


Merged &
\wstd{0.00}{0.00} & % SDV
\textbf{ \wstd{21.43}{1.10} } \\ % REaLTabFormer

% \midrule

% \multirow{3}{*}{
% Telstra } &

% Parent &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ & % REaLTabFormer

% Child &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ & % REaLTabFormer


% Merged &
% \wstd{*}{*} & % SDV
% \wstd{*}{*} \\ % REaLTabFormer

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> REaLTabFormer ArXiv/tables/results_ml_efficiency.tex <==
% ML efficacy results
\newcommand{\wstd}[2]{#1\small{$\scriptscriptstyle \pm \scriptstyle #2$}}
\newcommand{\bwstd}[2]{\textbf{#1}\small{$\scriptscriptstyle \pm \scriptstyle \mathbf{#2}$}}
\newcommand{\uwstd}[2]{\underline{#1\small{$\scriptscriptstyle \pm \scriptstyle #2$}}}

\begin{table*}[ht!]
\caption{Machine learning efficacy (MLE) and discriminator measure (DM) evaluated on the synthetic data generated by the models (columns) trained on six real-world datasets (rows): Abalone (AB), Adult income (AD), Buddy (BU), California housing (CA), Diabetes (DI), and Facebook Comments (FB). The MLE is measured by the $R^2$ for regression, while macro average $F_1$ is used for classification tasks; higher scores are better. A discriminator measure closer to 50\% is better. Best scores are highlighted for the MLE measure, considering standard deviation. No reported results for GReaT on the FB dataset due to impractical training time.}

\label{tab:mle-dm-results}
\vskip 0.1in
\begin{center}
\begin{small}
    \begin{tabular}{llcccccc}
        \toprule
         & & Original & TVAE & CTABGAN+ & Tab-DDPM & GReaT & \textbf{REaLTabFormer} \\
         \midrule
        
        \multirow{2}{*}{
        AB ($R^2$)} & 
        
        MLE ($\uparrow$) &
        \wstd{0.5562}{0.004} & % Original
        \wstd{0.3943}{0.012} & % TVAE
        \wstd{0.4697}{0.014} & % CTABGAN+
        \textbf{ \wstd{0.5248}{0.011} } & % Tab-DDPM
        % \wstd{0.2931}{0.018} & % distil-GReaT
        \wstd{0.3530}{0.031} & % GReaT
        \textbf{ \wstd{0.5035}{0.011} } \\ & % REaLTabFormer
        
        % \newcommand{\wstd}[2]{#1\small{$\pm$#2}}
        % \newcommand{\bwstd}[2]{\textbf{#1}\small{$\pm$\textbf{#2}}}
        % \newcommand{\uwstd}[2]{\underline{#1\small{$\pm$#2}}}
        
        % \newcommand{\wstd}[2]{#1\small{$\scriptscriptstyle \pm \scriptstyle#2$}}
        
        % \scriptscriptstyle \pm \scriptstyle .008
        
        DM \ \ ($\downarrow$) &
        - &  % \wstd{*}{0.00} & % Original
        \wstd{82.96}{2.42} & % TVAE
        \wstd{75.64}{1.20} & % CTABGAN+
        \wstd{59.88}{2.22} & % Tab-DDPM
        % \wstd{68.19}{0.48} & % distil-GReaT
        \wstd{70.46}{0.92} & % GReaT
        \wstd{63.08}{1.18} \\ % REaLTabFormer
        
        \midrule
        
        \multirow{2}{*}{
        AD ($F1$)} &
        
        MLE &
        \wstd{0.8155}{0.001} & % Original
        \wstd{0.7695}{0.004} & % TVAE
        \wstd{0.7778}{0.003} & % CTABGAN+
        \wstd{0.7922}{0.002} & % Tab-DDPM
        % \underline{ \wstd{0.7907}{0.003} } & % distil-GReaT
        \wstd{0.7997}{0.002} & % GReaT
        \textbf{\wstd{0.8113}{0.002}}\\ & % REaLTabFormer
        
        DM &
        - &  % \wstd{*}{0.00} & % Original
        \wstd{95.48}{1.34} & % TVAE
        \wstd{61.17}{0.40} & % CTABGAN+
        \wstd{53.73}{0.22} & % Tab-DDPM
        % \wstd{69.42}{0.29} & % distil-GReaT
        \wstd{68.04}{0.26} & % GReaT
        \wstd{55.78}{0.20} \\ % REaLTabFormer
        
        \midrule
        
        \multirow{2}{*}{
        BU ($F1$)} &
        
        MLE &
        \wstd{0.9303}{0.002} & % Original
        \textbf{ \wstd{0.9233}{0.002} } & % TVAE
        \textbf{ \wstd{0.9267}{0.002} } & % CTABGAN+
        \wstd{0.9057}{0.003} & % Tab-DDPM
        % \wstd{0.9272}{0.002} & % distil-GReaT
        \textbf{ \wstd{0.9279}{0.003} } & % GReaT
        \textbf{ \wstd{0.9278}{0.003} } \\ & % REaLTabFormer
        
        DM &
        - &  % \wstd{*}{0.00} & % Original
        \wstd{66.56}{0.56} & % TVAE
        \wstd{58.33}{0.49} & % CTABGAN+
        \wstd{54.43}{0.47} & % Tab-DDPM
        % \wstd{64.96}{0.41} & % distil-GReaT
        \wstd{62.18}{0.45} & % GReaT
        \wstd{55.86}{0.47} \\ % REaLTabFormer
        
        \midrule
        
        \multirow{2}{*}{
        CA ($R^2$)} &
        
        MLE &
        \wstd{0.8568}{0.001} & % Original
        \wstd{0.7373}{0.004} & % TVAE
        \wstd{0.5231}{0.006} & % CTABGAN+
        \textbf{ \wstd{0.8252}{0.002} } & % Tab-DDPM
        % \wstd{0.5416}{0.007} & % distil-GReaT
        \wstd{0.7189}{0.004} & % GReaT
        \wstd{0.8076}{0.003} \\ & % REaLTabFormer
        
        DM &
        - &  % \wstd{*}{0.00} & % Original
        % \wstd{62.06}{0.60} & % TVAE
        % \wstd{90.14}{1.03} & % CTABGAN+
        % \wstd{54.30}{0.89} & % Tab-DDPM
        % \underline{ \wstd{66.78}{0.47} } & % GReaT
        % \textbf{  \wstd{57.29}{0.56} } \\ % REaLTabFormer
        
        \wstd{62.06}{0.60} & % TVAE
        \wstd{90.14}{1.03} & % CTABGAN+
        \wstd{54.30}{0.89} & % Tab-DDPM
        \wstd{66.78}{0.47} & % GReaT
        \wstd{57.29}{0.56} \\ % REaLTabFormer
        
        \midrule
        
        \multirow{2}{*}{
        DI ($F1$)} &
        
        MLE &
        \wstd{0.7759}{0.014} & % Original
        \wstd{0.7395}{0.035} & % TVAE
        \wstd{0.7339}{0.024} & % CTABGAN+
        \wstd{0.7448}{0.031} & % Tab-DDPM
        % \wstd{0.4560}{0.064} & % distil-GReaT
        \wstd{0.7419}{0.03} & % GReaT
        \wstd{0.7315}{0.027} \\ & % REaLTabFormer
        
        DM &
        - &  % \wstd{*}{0.00} & % Original
        % \wstd{*}{0.01} & % TVAE
        % \wstd{*}{0.01} & % CTABGAN+
        % \wstd{*}{0.01} & % Tab-DDPM
        % \underline{ \wstd{*}{0.01} } & % GReaT
        % \textbf{  \wstd{*}{0.01} } \\ % REaLTabFormer
        
        \wstd{90.16}{1.31} & % TVAE
        \wstd{70.94}{1.99} & % CTABGAN+
        \wstd{69.00}{1.56} & % Tab-DDPM
        \wstd{74.88}{1.79} & % GReaT
        \wstd{75.56}{2.84} \\ % REaLTabFormer
        
        \midrule
        
        \multirow{2}{*}{
        FB ($R^2$)} &
        
        MLE &
        \wstd{0.8371}{0.001} & % Original
        \wstd{0.6374}{0.007} & % TVAE
        \wstd{0.4722}{0.053} & % CTABGAN+
        \wstd{0.6850}{0.006} & % Tab-DDPM
        % - & % distil-GReaT
        - & % GReaT
        \textbf{\wstd{0.7702}{0.004} }\\ & % REaLTabFormer
        
        DM &
        - &  % \wstd{*}{0.00} & % Original
        \wstd{97.72}{0.80} & % TVAE
        \wstd{93.60}{0.28} & % CTABGAN+
        \wstd{66.07}{0.23} & % Tab-DDPM
        % - & % distil-GReaT
        - & % GReaT
        \wstd{65.46}{0.83} \\ % REaLTabFormer
        % \textbf{  \wstd{*}{0.01} } \\ % REaLTabFormer
        
        % \midrule
        
        % \multirow{2}{*}{
        % CAR ($F1$)} &
        
        % MLE &
        % \wstd{*}{0.00} & % Original
        % \wstd{*}{0.00} & % TVAE
        % \wstd{*}{0.00} & % CTABGAN+
        % \wstd{*}{0.00} & % Tab-DDPM
        % \underline{ \wstd{*}{0.00} } & % GReaT
        % \textbf{\wstd{*}{0.00} }\\ & % REaLTabFormer
        
        % DM &
        % \wstd{*}{0.01} & % Original
        % \wstd{*}{0.01} & % TVAE
        % \wstd{*}{0.01} & % CTABGAN+
        % \wstd{*}{0.01} & % Tab-DDPM
        % \underline{ \wstd{*}{0.01} } & % GReaT
        % \textbf{  \wstd{*}{0.01} } \\ % REaLTabFormer
        
        \bottomrule
        
    \end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

